DMiner: Dashboard Design Mining and Recommendation

Dashboards, which comprise multiple views on a single display, help analyze and communicate multiple perspectives of data simultaneously. However, creating effective and elegant dashboards is challenging since it requires careful and logical arrangement and coordination of multiple visualizations. To solve the problem, we propose a data-driven approach for mining design rules from dashboards and automating dashboard organization. Specifically, we focus on two prominent aspects of the organization: arrangement, which describes the position, size, and layout of each view in the display space; and coordination, which indicates the interaction between pairwise views. We build a new dataset containing 854 dashboards crawled online, and develop feature engineering methods for describing the single views and view-wise relationships in terms of data, encoding, layout, and interactions. Further, we identify design rules among those features and develop a recommender for dashboard design. We demonstrate the usefulness of DMiner through an expert study and a user study. The expert study shows that our extracted design rules are reasonable and conform to the design practice of experts. Moreover, a comparative user study shows that our recommender could help automate dashboard organization and reach human-level performance. In summary, our work offers a promising starting point for design mining visualizations to build recommenders.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> src/sec6-recommendation.tex <==


\section{Recommender}
\label{sec: recommender}

In this section, we apply the extracted design patterns to the arrangement and coordination recommender, and conduct a comparative user study to evaluate the effectiveness of the extracted design patterns.

\subsection{Recommendation}
To demonstrate the usefulness of extracted decision rules, we develop a recommender that automates view arrangement and coordination.
Specifically, given $n$ views, the recommender aims to provide arrangement and coordination that best aligns with the design patterns.

\autoref{fig: recommendation} provides an overview of the recommender pipeline.
It takes the common method in optimization-based visualization recommenders, that is, to enumerate possible designs and recommend designs with the highest scores~\cite{wu2021ai4vis}.
Specifically, it firstly enumerates all possible arrangements (\ie~positions and sizes for each view) to generate candidates.
Then it computes the score for each candidate by checking whether it obeys or violates the extracted decision rules.
Inspired by~\cite{moritz2018formalizing}, the cost score is a weighted sum of violated decision rules.
We use the importance of each decision rule as the weight, which measures how the rule is important to the prediction.

However, it is time-consuming and infeasible to calculate scores for all candidates.
The number of possible candidates is huge since it grows exponentially with the number of views.
To reduce the computational complexity, we adopt the common strategy in previous studies on visualization recommendation (\eg SeeDB~\cite{vartak2015seedb} and QuickInsights~\cite{ding2019quickinsights}), \ie~pruning, to balance the efficiency and performance.
We first consider the \textbf{S2S} patterns (\ie~single-view data encoding features to single-view layout arrangement features), since it only considers single view and therefore has smaller complexity than pairwise-view computations.
We use cost scores computed from \textbf{S2S} patterns to get the top 1\% results, which are subsequently fed into the next step, \ie~to compute scores based on all other patterns.
The number 1\% is decided on an empirical basis to reduce the running time to seconds, which is desirable in real-world scenarios. 
Finally, we recommend the arrangement and coordination with the highest score.


% Our recommendation framework is summarized on the \autoref{fig: recommendation}.
% Given $n$ views to create a dashboard, we firstly enumerate all possible arrangements for the given $n$.
% \aoyu{cannot understand ``display space'', ``rectangles'' and ``memory searching''. If they are terms, need to add explanations with references.}
% Specifically, we have limited the size of each view as rectangles in \autoref{sec:overview}.
% Thus, we formulate this enumeration problem as dividing the display space of a dashboard into $n$ rectangles, then adopting dynamic programming to recursively find every next possible rectangles given the previous selected rectangles~\cite{bellman1966dynamic}.
% The detail of this algorithm is provided in the \yanna{Supplementary S3}.
% For each potential arrangement, we permute the views to generate all arrangement candidates.
% Then we check how each candidate obey or disobey the patterns extracted in \autoref{sec:design_patterns}. 
% While the candidate obeys one specific pattern, then it will get the corresponding importance as its score.
% And if the candidate breaks the pattern, it will get 0.
% In this case, we can get the score of all candidates, and recommend the one with the highest score.

% However, it is time-consuming and infeasible to calculate scores considering all patterns for all arrangement candidates.
% And there are some reasons.
% Firstly, the number of potential arrangements increases exponentially with the number of views.
% And it will increase by $n!$ times due to the permutation and combination of view for each arrangement.
% What's more, the number of view pairs, \ie~$n*(n-1)$, further worse the case.

% In this paper, we adopt the common strategy in previous studies on visualization recommendation (\eg SeeDB~\cite{vartak2015seedb} and QuickInsights~\cite{ding2019quickinsights}), \ie~pruning, to balance the efficiency and performance.
% We firstly only consider the \textbf{S2S} patterns, since it consider each view as individuals and ignored the interrelations. 
% Then, we check how each candidate obey the \textbf{S2S} patterns and calculate the score for them.
% To increase the arrangement diversity, we group the candidates with same arrangement but different view permutation as one and rank them according to their average score.
% Then, we filter the top $maximum(1\% \times \# \ arrangements, 10)$ arrangements. \yanna{how to describe this number without formula -.-}
% This means that we will take at least $10\times n!$ candidates.
% Following the similar process, we further calculate the score for each filtered candidates considering all other patterns.
% Specifically, for the coordination, we also adopts the enumeration methods, \ie~trying every coordination type for each pair and finally selecting the one with highest score.
% Finally, we recommend the arrangement and coordination with the highest score.

\iffalse
Given such set of views, we firstly regard it as $n$ independent views and $n * (n-1)$ view pairs.
Then we extract the corresponding $n$ sets of $SF_{D\&E,i}$ features and $n * (n-1)$ sets of $SF_{D\&ER,(i, j)}$ features by conducting the feature extraction and feature processing described in \autoref{sec: feature_extraction} and  \autoref{sec:design_patterns}.
For each individual view and view pairs, we can infer the \textit{mapped target} is true or false of each  pattern based on their data and encoding features.
For example, for a view $i$, we can infer its $SF_{Arr, i}$ by observing whether the $SF_{D\&E,i}$ features obey the \textit{conditions} of the \textbf{S$\rightarrow$S} pattern or not.
If $view \ i$ obeys the condition of a pattern,  the corresponding \textit{mapped target} tends to be true, since the coefficients of all the patterns are positive.
We denote the inferred \textit{mapped target} for $view \ i$ as $\tilde{Y}_{view \ i} = \{y_1, y_2, ..., y_k\}$, where $y_j \in \{0, 1\}$.
However, this forwarding inference has some limitation since there may be some conflicts between views.
For example, view $A$ and view $B$ are all preferred to be on the top left position.
Thus, the final arrangement and coordination must break some design patterns, and our goal is to recommend those with best overall score. 

To achieve this goal, we adopt the brute-force and greedy algorithm.
We firstly brute-force all potential arrangements for the given number of views $n$.
We formulate this problem as dividing the display space into $n$ rectangles, then using memory searching to recursively find every possible rectangles given the previous selected rectangles.
The details can refer to the Supplementary xxx.
And to remove some inappropriate division, we calculate the distribution of \textbf{aspect ratio with the number of views} \yanna{how to describe aspect ratio $\times$ the number of views}, and remove those aspect ratio with the number of views above the 95th percentile or below the 5th percentile (should we need to clarify this one?).
In this case, we get 200 kinds of divisions for $n=5$, while 1392 for $n=6$.
The number of divisions increase exponentially with the number of views.
And it will increase by $n!$ times due to the permutation and combination of view for each division, \ie~ there will up to $200 \times 5! = 24000$ arrangement candidates for $n=5$.
And each candidates need to consider $n$ single-view relations (\ie~S2S) and $5*n*(n-1)$ other pair-related relations.
% Especially for coordination type, you need to try 3 potentials for each pair.
Thus, it is time-consuming to calculate scores considering all relations for all arrangement candidates.

To make the trade-offs between
the performance and efficiency, we adopts greedy algorithm by firstly filtering some arrangement candidates with higher score considering only the \textbf{S2S} relation, and then applying all other relations.
We only consider the \textbf{S2S} relation, since it consider each view as individuals and ignored the interrelations. 
Specifically, for each arrangement candidates, we can conduct the same process to extract the $SF_{Arr, i}$.
We then convert the $SF_{Arr, i}$ features to vectors aligning the  prediction target order of $S2S$ relations.
Then, we can get the arrangement features for $c$th arrangement candidate as $Y_{candidate \ c} = \{y_1, y_2, ..., y_k\}$.
Thus, for $view \ i$ arranging in $c$th arrangement candidate, we can get the score as: 
\begin{equation}
\begin{aligned}
\centering
S_{view \ i, candidate \ c}= w^T (\tilde{Y}_{view \ i} \odot Y_{candidate \ c}), 
\end{aligned}
\end{equation}
where the $\odot$ is inclusive or, \ie~1 for two same elements and 0  for two different ones.
Same elements means that the $c$th arrangement candidate is aligned well with what the design patterns predicted.
Thus, the $c$th arrangement candidate gets the corresponding scores for obeying the proposed patterns.
Considering the number of views is $n$, the whole score for $c$th arrangement candidate is the sum of the score of all individual view:
\begin{equation}
\begin{aligned}
\centering
S_c  = \Sigma_{i=1}^{n} S_{view \ i, candidate \ c}, 
\end{aligned}
\end{equation}

In this case, we get the score of each arrangement candidate considering \textbf{S2S} relations.
To increase the arrangement diversity, we group the candidates with same rectangle division but different view combinations as one and consider their average score as the final score.
Then, we select the $maximum(1\% \times \# \ divisions, 10)$ divisions with largest average score.
This means that we will take at least $10\times n!$ candidates.
Following the similar process, we further calculate the score for each filtered candidates considering all other relations.
Specifically, for the coordination, we also adopts the brute-force methods, \ie~trying every coordination type for each pair and finally selecting the one with highest score.
Finally, we recommend arrangement and coordination with the highest score for the given $n$ views.


We have tried another greedy algorithm, that is, every time we find a position for a view with the highest score. 
Though efficiently, xxxx.
\yanna{need to re-consider the reason}
% \textbf{Though efficiently, it has a worse result.}
Thus, we chose the first choice.
\fi


%  Greedy algorithm
% \begin{algorithm} 
%  \caption{Calculate All Possible Partition} 
%  \label{alg:memory_search} 
%  \begin{algorithmic}
%   \Require \#Grid $g$, \#Views $n$, \# Result $res$  
%   \Ensure List of Position List $P_L$
%   \Function{DivideSpace} {$g, n, res$}
%   \State $ status \gets g*g \  array \  filled \  by \  0 $
%   \State $startX \gets 0$ 
%   \State $startY \gets 0$ 
%   \State $posList \gets []$
  
%   \State $calPosList(status, startX, startY, n, g, posList, res)$
%   \State {Return $res$}
%   \EndFunction
%   \Function{calPosList} {$status, startX, startY, viewNum, gridNum, posList, res$}
%   \If {$len(posList) == viewNum$}
%     \If {$status$ are all 1}
%     \State $res.append(posList)$
%     \Else 
%     \State {Return ;}
%     \EndIf
%   \EndIf
%     \For {$width=1 \to gridNum$}
%     \For {$height=1 \to gridNum$}
%       \State {$newPos = [startX, startY, width, height]$}
%       \If {the $newPos$ region of $status$ are all 0}
%       \State {$newPosList = posList + [newPos]$}
%       \State {$newStatus$ = set $newPos$ region of $status$ to 1}
%       \State {$startX, startY$ = first upper left 0 of $newStatus$ }
%         \State {$calPosList(newStatus, startX, startY, viewNum,$}
%         \State {\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \  $gridNum, newPosList, res)$}
%       \EndIf
%     \EndFor
%     \EndFor
%     \EndFunction
%  \end{algorithmic} 
% \end{algorithm}

\begin{figure*}
    \centering
    \includegraphics[width=1\linewidth]{figures/Result.pdf}
    % \vspace{-0.25in}
    \caption{An overview of the study result. 
    Specifically, each column describes the score of a metric in three groups, \ie~the group considering all dashboards, the group with 3- and 4-view dashboards, and the group with 5- to 8-view dashboards.
    And six metrics cover 3 perspectives, \ie~arrangement, coordination, and overall (\ie~both).
    Each sub-plot presents the score of 5 recommendations regarding the corresponding metric and group.
    Here, we show some results from 3 metric perspectives:
    (1) \textbf{Arrangement}: For dashboards with 5-8 views, \textit{Human} performs significantly better than all others in three arrangement metrics, except that the \textit{Full} recommendation achieves similar results in terms of the arrangement logic and helpful to analyze.
    (2) \textbf{Coordination}: \textit{Default} without coordination receives a significantly worse result than others. And our \textit{Full} and \textit{Partial} recommendations achieve significantly better performance than \textit{Human}, considering all dashboards and the dashboards with 3-4 views.
    (3) \textbf{Overall}: \textit{Full} recommendation suppresses \textit{Human} regarding dashboards with 3-4 views, and achieves \textit{Human}-like performance considering all dashboards and dashboards with 5-8 views.}
    \label{fig:result}
    \vspace{-1em}
\end{figure*}


\subsection{User Study}
\label{sec: user study}
To verify the effectiveness of our recommender which is based on learned design patterns, we conducted a user study with novice dashboard users. 
% This section introduces the participants, the procedure and the results of the user study.

\paragraph{Participants.} 
% We recruited 12 participants (9 females, 3 males, age: $24.8 \pm 1.76$) in the study.
% Most participants are PhD or MSc students from diverse background, like finance, knowledge base, data mining, human-computer interaction,  and recommendation system, while one participant is the data analysts in a finance company.
% Given a 7-point Likert scale, they were experienced in the data analysis ($\mu = 5.25 , \sigma = 0.45$).
In this study, we recruited 12 participants (9 females and 3 males, ages 22 to 27, with an average of $24.8$). 
They are all well educated (7 Ph.D. students, 3 MSc students, 1 research assistant, and 1 data analyst) and from diverse backgrounds, including visualization (4), finance (2), recommendation system (1), human-computer interaction (2) and data science (3). 
All the participants are reported as experienced in the data analysis by giving a 7-point Likert scale ($\mu = 5.25, \sigma = 0.45$). 
Each participant was compensated with \$10 after finishing the user study.

% \textbf{Datasets and settings.}
% In our user study, we chose 15 representative dashboards to participants.
% The dashboards cover almost all of the mark types (11/13), and are from various topics, like terrorist attack, business, ride bike, auto policy, product sales, and patients.
% What's more, the number of views ranging from 3 to 8, obeying the distribution proposed by \cite{al2019towards}, \ie~3- and 4-view dashboards are the most common, followed by the 2-, 5- and 6-view, while the 7- and 8-view are less.
% Considering that the arrangements for 2-view dashboard are limited and so as the 3-view, we finally select four 4-view dashboards views, three each for the 3-, 5-, and 6-view, and one each for the 7- and 8-view.
% The user study lasts about 1 hour for each participant. 
% Before the user study, we ask for the consents for recording the whole user study process and their comments.
% And then, we conduct a brief 5-min introduction of our work.
% After that, the participants are asked to scoring the arrangement and cooridnation of 5 dashboards selected from the whole 15 dashboards and are encouraged to think aloud about why give the corresponding score.
% Thus, each dashboard will be evaluated by 4 participants.
% And for each dashboard, 5 recommendations are provided:
% \begin{itemize}
%     \item \textit{Baseline} recommendation is the default organization provided by the Tableau, where next view will evenly split the left-top largest view, but do not recommend any coordination among views;
%     \item \textit{Origin} recommendation is created by the human;
%     \item \textit{Basic} recommendation only considers the organization of each individual view, \ie~just using \textbf{S2S} relations;
%     \item \textit{Partial} recommendation considers all patterns except those about interrelations between arrangement and coordination; and 
%     \item \textit{Full} recommendation leverages all design patterns.
% \end{itemize}

% At the beginning of each dashboard evaluation, we let users to know about each visualization that needs to be arranged.
% We will explain to the participants when they have any problems in understanding.
% When they feel they have grasped the content of the visualizations, we will show the corresponding 5 recommendations one-by-one with random order.
% The participants freely interact with them and explain the disadvantages and advantages. Then they finish the 7-point Likert scale questions regarding the arrangement (including logic, aesthetics, and the ability to help analyze data), coordination (including logic, and the ability to help facilitate exploring data), and the overall score.
% Thus, they will be $12(participants) * 5 (dashboards) * 5(recommendations) * 6 (metrics) = 1800$ scores.

% \fzz{Zezheng's advice:----------------------------------------------------}

\paragraph{Dataset.}
In the user study, 15 representative dashboards with four recommended variants were presented to the participants for scoring.
Despite the dashboard created by \textit{Human}, the four recommended variants are:
\begin{itemize}
    \item \textit{Default}: the default recommended dashboard by Tableau~\cite{tableau}. One point to mention is that the default dashboards do not have coordination since Tableau does not support the recommendation of coordination;
    \item \textit{Basic}: the recommended dashboard using only \textbf{S2S} patterns;
    \item \textit{Partial}: the recommended dashboard considering all patterns except those about interrelations between arrangement and coordination; and 
    \item \textit{Full}: the recommended dashboard leveraging all design patterns.
\end{itemize}
For simplicity, each original dashboard with four variants is called \textit{a group of dashboards}.
Therefore, we totally have 15 groups of dashboards for participants' scoring.
The dashboards cover almost all of the mark types (10/13), and are about various topics, like business and patient analysis. 
What's more, the number of views ranges from 3 to 8, obeying the distribution in \autoref{fig:basic_info} \cc{A}. 



\paragraph{Procedure.}~The user study lasted about 1 hour, and we asked for participants' consent for recording the whole user study. 
Before the user study, we conducted a 5-minute introduction of our work.
In the user study, each participant was asked to score the arrangement and coordination of 5 groups of dashboards sampled from the 15 groups. As a result, each group of dashboards is evaluated by 4 participants. 
Before evaluating each group of dashboards, we introduced each view that needs to be arranged. 
When the participants felt familiar with the views, they freely explored the dashboards.
After the free exploration, they were asked to score the dashboards using the 7-point Likert scale.
They were asked to score arrangement (including logic, aesthetics, and the ability to help analyze data), coordination (including logic and the ability to help facilitate exploring data), and the overall score,  which refers to the previous studies~\cite{smith2013data, wang2019datashot}. Specifically, the ``logic" measures how well the arrangement and coordination follow a human's ``logical" analysis~\cite{dowding2018development}.
All the participants were encouraged to think aloud about why they gave the corresponding score. 
% After the user study, we conduct an interview about 
% \haotian{Please see my comments.}








% \fzz{---------------------------------------------end Zezheng's advice}


% \textbf{Hypotheses}. We anticipate that the recommendation will perform better with considering more features, and the performance of \textit{Full} mode will close to human's performance while better than baseline's in both the arrangement and the coordination. 
% Thus, we formulated the following hypotheses:
% first, the \textit{Full} recommendation mode will perform better than the \textit{Partial} and the \textit{Basic} recommendation, in terms of the arrangement (\textbf{H1}), coordination  (\textbf{H2}), and both(\textbf{H3}).
% Secondly, the effectiveness of \textit{Full} recommendation will close to that of human, in terms of the arrangement (\textbf{H4}), coordination  (\textbf{H5}), and both(\textbf{H6}).
% Thirdly, \textit{Full} recommendation will have great difference to the \textit{Baseline} in terms of the arrangement (\textbf{H7}), coordination  (\textbf{H8}), and both(\textbf{H9}).

\subsubsection{Quantitative Analysis}







% \input{tables/userStudy_table}



This section introduces and discusses the quantitative results of our user study.
To analyze the results, we further split all dashboards into two groups according to the number of views in dashboards, \ie~the dashboards containing 3-4 views and the dashboards containing 5-8 views.
The rationale for the split stems from the feedback from our participants.
% They mentioned that their focus on dashboards arrangement and coordination depends on the number of views.
% Specifically, \
They indicated that they care more about the arrangement and coordination when the number of views is more than 4 since a well-organized dashboard reduces their cognitive load of viewing many visualizations.
Figure~\ref{fig:result} presents the average ratings of recommended dashboards using six metrics.
To further analyze the results, we performed the one-way ANOVA (5 recommendations) on 6 metrics between the dashboards with different numbers of views. In the following, we will introduce the result regarding arrangement, coordination, and overall.
% When conducting user study, many participants mentioned that when there are less number of views, the relationship of view is simple and they almost can understand the dashboard at a glance.
% and the arrangement mostly is feasible and clear.
% While when it comes to more views, they need to analyze the relationship among views to understand the dashboard.
% so the arrangement will be very crucial for understanding.
% Inspired by this, we split the dashboards into two partitions, \ie~the 3- and 4-view, and the 5- to 8-view.
% Thus we have totally 3 groups, \ie~ all-view group, 3- and 4-view group, and the 5- to 8-view group.
% In this section, we will introduce the result and our findings in terms of the arrangement, coordination, and overall considering both across 3 groups.

\begin{figure*}[!ht]
    \centering
    \includegraphics[width=1\linewidth]{figures/positive_example.pdf}
    % \vspace{-0.25in}
    \caption{A case identified in our user study. \cc{A} and \cc{B} are the dashboards created by \textit{Human} and our \textit{Full} recommendation, respectively. Our recommended dashboard is highly rated due to outstanding logic and coordination (see \cc{A5} and \cc{B5}).
    Participants recognized that the \cc{B1} is more suitable than \cc{A1} to act as a starting point to explore the dashboard.
    And for the same view pair, our recommended coordination type is \textit{Brush}, which keeps the context for comparison.
    However, \textit{Human} chooses \textit{Filter}, which leads to a change in the display and can confuse the users.}
    \label{fig: positive_example}
    % \vspace{-2em}
\end{figure*}

\textbf{Arrangement}.
% First, we would like to discuss the findings regarding arrangement of views in dashboards.
For all dashboards regardless of view numbers, no significant difference is observed among 5 recommendations for all three perspectives, \ie~logic, aesthetics, and ability to help analyze data.
While for dashboards with 3-4 views, we still cannot observe any significant differences among the 5 recommendations. 
And we can notice that the \textit{Full} has a slightly higher score than \textit{Human}.
\autoref{fig: positive_example} provides one example, where \cc{A} is created by \textit{Human} and \cc{B} is our \textit{Full} recommendation.
Participants recognized that the position logic of \cc{B} is better than  \cc{A}, since \cc{B1} is more suitable than \cc{A1} to act as a starting point to guide the data analysis.
And the symmetrical position of \cc{B2} and \cc{B4} are also plausible.
However, they thought our \cc{B1} (map) should be with a higher height, but still better than \cc{A1}, where the bar with a too larger height.
What's more,  we can notice that the \textit{Default} has a higher score in terms of all three arrangement metrics.
This is probably  because the \textit{Default} divides the largest view into two even views each time, resulting in a  balanced aspect ratio and a neat arrangement.
The participants prefer such a balanced arrangement, especially when there are relatively less views and their interrelations are simple. 


While for dashboards with 5-8 views, \textit{Human} recommendation significantly differs from all others. 
The only exception is the \textit{Full} recommendation in terms of the logic and the ability to help analyze data.
% while \textit{Human} are significantly more aesthetically pleasing than all others including the \textit{Full}.
Participants recognized that the position recommended by our \textit{Full} mode is logically plausible. 
However, it sometimes has problematic sizes, \ie~too small or too large height or width to cause deformation and extrusion, such as \autoref{fig: negative_example} \cc{B2}.
Thus, it led to a slightly lower score on the logic but a great performance drop on the aesthetics. 
Moreover, the problematic size does not greatly influence the ability to help understand since the position is more important.
What's more, both \textit{Full} and \textit{Partial} recommendations perform significantly better than \textit{Default} in terms of the logic and the ability to help analyze.
This may be attributed to that \textit{Default} arranges the views according to the alphabetical order by view name, leading to the worse logic confusing the participants.
Furthermore, though \textit{Default} still recommends the arrangement with the balanced aspect ratio, it suffers the same deformation and extrusion problems as our three recommendations. 
P8 has mentioned that ``\textit{when there are too many views, there should be a dominant one telling me what it wants to express. 
The exactly equal size confuses me.
And it is challenging for me to identify what I should pay attention to first}."
P9 had similar comments.
This may be the main reason why ours are slightly better in aesthetics, and significantly better in the logic and ability to help analyze than the \textit{Default}.

What's more, we further notice that, among our three recommendations, \textit{Full} achieves the best arrangement performance, followed by \textit{Partial} and \textit{Basic}.
\textit{Basic} is the worst among our three recommendations and only slightly better than the \textit{Default} for the dashboards with 5-8 views.
While \textit{Partial} is better than \textit{Basic}, it has a great difference from \textit{Default} in terms of the logic and the powers to help analyze, and it even achieves human-like logic.
And \textit{Full} is better than \textit{Partial}, and its arrangement achieves not only human-like logic but also human-like powers to help analyze. 

\textbf{Coordination.}
Since \textit{Default} has no coordination, it has significantly worse results than all other recommendations in terms of both logic and the ability to facilitate exploration.
P1 mentioned that ``\textit{Without coordination, it was challenging for me to identify the related data cross views and focus the data of interest}".
P2 commented that ``\textit{The views without any interaction are really like a decoration, and it is strange to composite such views with others}."
What's more, \textit{Full} and \textit{Partial} recommendations possess significant differences to \textit{Human} among all dashboards and dashboards with 3-4 views.
This may be because we recommend either \textit{Brush} or \textit{Filter} for almost all view pairs.
As shown in \autoref{fig:basic_info} \cc{D}, our three recommendations recommend  more coordination than \textit{Human}.
And participants prefer comprehensive coordination, since it gives a stronger power of exploration.
What's more, P5 and P11 appreciate our recommendation of the interaction type.
As shown in \autoref{fig:basic_info} \cc{D}, 
\textit{Human} recommendation prefers the  \textit{Filter}  rather than \textit{Brush}.
And participants thought our \textit{Brush} recommendation was more appropriate in some cases, since it does not change the context and enables comparisons.
For example, in \autoref{fig: positive_example}, \cc{A5} is the filtered result of \cc{A2}, while \cc{B5} is the brushed result of \cc{B4}, and \cc{B5} keeps the context well to compare.
When it comes to dashboards with 5-8 views, \textit{Full} and \textit{Partial} have no significant difference from \textit{Human}, while \textit{Human} gets a very high score.
This is because when more views are involved, participants are not just concerned with the completeness of coordination; they recognised that a clearer logic of coordination is more important.
P7 said, ``\textit{Too many coordination relationships will confuse me.
One view will lead to the change of lots of views, and I do not know where to look.}"
In this perspective, most of the \textit{Human} dashboards are more appropriate, while our \textit{Full} recommendation provides a more suitable coordination type.

For our three recommendations, \textit{Full} and \textit{Partial} achieve almost the same performance and are better than \textit{Basic}.
When it comes to the dashboards with 3-4 views, \textit{Basic} performs significantly better than \textit{Human} in terms of both the coordination logic and the power to facilitate exploration.
However, the coordination logic of \textit{Human} suppresses \textit{Basic} when there are at least 5 views, and they are almost the same for all dashboards regardless of the number of views.



\textbf{Overall.}
Though \textit{Default} achieves similar arrangement performance to other recommendations, it gets a significantly worse result due to the lack of coordination across 3 groups.
Participants all recognized the indispensability of the coordination.
For the all-view group, \textit{Full} has a slightly but not significantly better overall score than the \textit{Human},
though \textit{Full} has a significantly great coordination score to the \textit{Human}.
This is because the participants thought that the arrangement was slightly more important than the coordination for data analysis.
And for 3- and 4-view dashboards, \textit{Full} is significantly better than the \textit{Human}, due to a similar result in arrangement but better and more comprehensive coordination provided \textit{Full}.
While for 5- to 8-view group, the \textit{Full} still achieves human-like performance.
And our 3 recommendations have no significant difference from each other.


% \textbf{In summary, xxxx.}

In summary, we earn nice feedback about our recommendations from participants.
% Participants appreciated our recommendations for both the arrangement and coordination, 
% with average score of 5.56 and 5.67 respectively.
Participants appreciated the automating results for both the arrangement and coordination. 
And P11 expected that our recommendations can combine to her work, ``\textit{I really love this work, and I hope it can be integrated into my workflow, ..., I believe it will greatly facilitate my analysis process.}"
However, our approach occasionally provides some unreasonable recommendation.
\autoref{fig: negative_example} illustrates a case where \cc{B} recommended by our \textit{Full} mode got a low score in the user study.
And \cc{A} is created by human.
Specifically, the participants' confusion mainly came from three perspectives: 1) the \cc{B2} was inserted between two similar views; 2) the size of \cc{B2} is too small to show the details; 3) \cc{B1} about the ``winter" is on the top of \cc{B2} about the ``summer". 
% \yanna{should we provide the reason to explain this?}
% \yanna{Maybe we can remove the \autoref{fig: negative_example} \cc{A}}
% \yanna{Check the why it split to } 



% They get inspiration from the recommendation ($\mu = 6.22$). 
% P8 mentioned that ``\textit{Some arrangements really surprise me since I never think of this, and I can get some inspiration to arrange}". 
% And they appreciated the automating results.
% P11 expected that our recommendations can combine to her work, ``\textit{I really love this work, and I hope it can be integrated into my workflow, ..., I believe it will greatly facilitate my analysis process.}"




% Since we do not consider the details of data attributes, \eg~ the number bar in the x-axis or y-axis, leading to the visual congestion and the unclear details.
% After finishing the user study, we refer to the size of the view in original dashboards and try to make a improvement of the original arrangement.
% The details can be seen on the Supplementary xxx.

\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{figures/negative_example.pdf}
    % \vspace{-0.25in}
    \caption{A case identified in our user study. 
    \cc{A} is created by \textit{Human}, while \cc{B} is created by our \textit{Full} recommendation. 
    Compared to the original dashboard, the recommended one received a lower score and our participants pointed out that the problematic arrangement from 3 perspectives, \ie two similar views \cc{B1} and \cc{B3} are not positioned together, too small in size of \cc{B2}, and \cc{B1} about ``winter" is on top of the  \cc{B3} about ``summer".}
    \label{fig: negative_example}
    % \vspace{-2em}
\end{figure}

\subsubsection{Design Suggestions}
% We summarized several design suggestions based on participants' feedback during the user study.
Combining the feedback from the participants and the findings from the unreasonable recommendations, we summarized the following design suggestions, which supplement our proposed method.


\textbf{Arranging views by proximity.}
All participants commented that views encoding similar information or the same chart types should be positioned closely with equal sizes, such as   \cc{A1} and \cc{A2} in \autoref{fig: negative_example}.
This perspective confirms the proximity principle in visual designs that elements near each other are perceived as related.
We encourage future research to investigate the effects of view proximity on their layout arrangement through empirical experiments.
% \yanna{should we call back the \autoref{fig:case example} \cc{3}?}

% This is the result of not considering the number of attributes show in the horizontal and vertical axis.
% \textbf{Similar views should put closely or put symmetrically and be equipped with same coordination.}
% All participant recognized that views encoding similar information or in similar visual type should be position closely and has the same size.
% % And they can accept the symmetrical arrangements.
% P8 further noticed that, ``\textit{similar view should be equipped with same coordination.}"
% P8 argues that if two views has exactly same meaning and importance (such a map showing origin station and a map showing destination station), it is better that two views raise and receive exactly same interaction to others.

\textbf{Reducing view ``islands''.}
Most participants mentioned that it was less describable to have a view that was an ``island'' and disconnected with other views in terms of encoded attributes or coordination.
Instead, the dashboard should compose views as a cohesive whole.
Furthermore, P10 expected the dominant view to be coordinated with the remaining views.
This comment echoed that of P12, ``\textit{the top-left most view is an overview, but it is strange that there is no coordination. It should guide me to explore other views.}" 
% and P12 comments one recommendation that, ``\textit{the top-left most view is an overview but it is really strange that there is no coordination raised by it. It should guide me to explore}". 
This comment aligns well with one of the patterns mentioned in \autoref{sec:case_study}.

% \textbf{Only one connected components.}
% Most participants mentioned that it will be strange that there are some views totally separated with other views, \ie~ the view without any coordination.
% P6 expected that ``\textit{there is only one connected component for each dashboard}".
% The concept of connected component refer to the graph domain, which represents that there are at least one coordination linking one view to others in the same component.
% While there is not any coordination between different connected components.
% Thus, more than one connected component means that there are some parts of dashboard did not interact with each other.
% With only one connected component ensures that the views in a dashboard are a cohesive whole.
% What's more, P10 expected that the dominant view must have coordination, and P12 comments one recommendation that, ``\textit{the top-left most view is an overview but it is really strange that there is no coordination raised by it. It should guide me to explore}". 
% This comment aligns well with one of the patterns mentioned in \autoref{sec:case_study}.

\textbf{Adding cues or hints for coordination.}
Participants commented that it was difficult to find coordination among views. 
They need to carefully explore each view and observe other views to identify whether there is coordination between them.
This process is tedious and poses high cognitive loads.
Thus, it is important to provide user-friendly hints on coordination among views.

% \textbf{The explicit visual cue for coordination.}
% During the user study, many participants complain that they need to explore every view and observe other views carefully to identify whether there are coordination between them or not.
% This process is really tedious and requires them to remember and observe what had happened, which is very unfriendly.
% They expected we can provide some friendly explicit visual cues among coordination.

\textbf{Considering the semantics.}
Participants deemed semantics as an important concern in arranging views.
For instance, P1 said ``\textit{the view about peak hour in summer month should on the top of that in winter}", (a counter example shown in \autoref{fig: negative_example} \cc{B1} and \cc{B3})
This requires understanding the semantic meaning of each view and their ``orders''.
However, visualization sequencing remains a challenging problem that warrants future research~\cite{lin2020dziban}.

% \textbf{Consider the semantics.}
% Most participants preferred those arrangement the view with overview information at the top or on the left.
% They believed this was in line with analytical habits of human, and it provides a clear starting point to analysis.
% And they prefer to consider those simple view \yanna{\ie~using less fields} as overview, which aligns well with one of our extracted patterns, shown in \autoref{fig:case example} \cc{4}.
% What's more, for some views in chronological order, participants proposed that these views should align with the common sense.
% \yanna{In \autoref{fig: examples} \cc{C} and \cc{D},}
% P1 and P3 said, ``\textit{the view about peak hour in summer month should on the top of the view about peak hour in winter month, thus the \cc{C} has better logic than \cc{D} }".
% P3 further confirmed that the views with important information should have the larger size, like balance in the bank customer analysis.
% \aoyu{Need more information: do not understand, e.g., what is ``simple view as overview'', ``common sense'', `` view about discharge'', etc.}
% \yanna{how about now? Is it better?}

\textbf{Paying attention to cross-view filtering.}
Participants noted that cross-view filters could result in a huge difference in the filtered view (\eg~ \cc{A1} leading to a large change from \cc{A2} to \cc{A5} in \autoref{fig: positive_example}).
Such changes catch attention but also bring about a cognitive load.
For example, P1 said, ``\textit{I got lost for seconds, wondering what makes the sudden change. It is a waste of time since I soon realize the reason, and it does not bring new data insights.}''
This problem suggests the need for careful consideration of cross-view filtering.


% \textbf{Filter for overloaded information, and Brush for non-overloaded information.}
% During the user study, participants notices that filter will lead to a large change of the dashboard content and disable the comparison.
% P5 and P11 both mentioned that \textit{filter} is suitable for filtering the data of interest when encountering overloaded information, such as the text table with thousands of lines of text; while if there are less information shown clear,  \textbf{brush} is more suitable.
% \aoyu{Need more information: what does it mean by ``filter'' will ``disable the comparison''? Is this good or bad? If it is bad, why ``Filter for overloaded information''?}
% \yanna{like \autoref{fig: user_study_examples} \cc{A1}}


==> tables/problematic_rule4.tex <==
\begin{table}[!h]
\caption{This tables shows five rules with average score less than 3. Most of them are related to predicting the arrangement features and data features (\ie~ordinal filed).}
\label{tab:problematic_rules_4}
\centering
\begin{tabular}{p{7.5cm}|p{0.7cm}}
\hline
\textbf{Rule}                                                                                                                                   & \textbf{Score} \\ \hline
If view A highlights view B, then view A has height or width as 3 or 4.                                                            & 3.5            \\ \hline
If view A doesn't have fields on X-axis, then view A has width as 1.                                                                    & 3.5            \\ \hline
If view A is \textit{Circle}, and has fields on X-axis, then view A is on x=3.                                                                  & 3.5            \\ \hline
If view A and view B encode the same fields on color, and they have different fields on Y-axis, then view A or view B has height as 3. & 3.25           \\ \hline
If view A is \textit{Text}, and view B has fields on Y-axis, the distance between A and B is larger than 2.                                              & 3.25           \\ \hline
If view A highlights view B, then view A is on y=1, or occupies grid1\_3, or grid3\_0, or grid3\_3.                                         & 3              \\ \hline
If view A and view B have unequal number of fields on Y-axis, then view A or view B is on y=3.                                                  & 3              \\ \hline
If view A and view B have no common fields, and they don't have fields on X-axis,then view B is on x=3.                             & 3              \\ \hline
If view A is \textit{Map}, and view A has more than 1 ordinal field, then view A is on x=2.                                                            & 2.75           \\ \hline
If view A is not \textit{Bar}, and view A has more than 1 ordinal field, then view A is on y=3.                                                        & 2.75           \\ \hline
If view A is \textit{Text}, and view B has no fields on Y-axis, then view B is on the left of view A.                                            & 2.75           \\ \hline
If view A has no fields on Y-axis and has ordinal fields, then view A is on y=1.                                                    & 2.75           \\ \hline
If view A shares some common and some different fields on Y-axis with view B, the view B is on y=1.                                          & 2.67           \\ \hline
\end{tabular}
\end{table}

==> tables/userStudy_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table*}[]
\begin{tabular}{c|ccc|ccc|ccc}
\hline
                      & \multicolumn{3}{c|}{\textbf{Layout Logic}}                                    & \multicolumn{3}{c|}{\textbf{Layout Aesthetics}}                                  & \multicolumn{3}{c}{\textbf{Layout Helpful to Analyze}}                           \\ \hline
                      & \multicolumn{1}{c|}{All}  & \multicolumn{1}{c|}{3- and 4-view} & 5- to 8-view & \multicolumn{1}{c|}{All}     & \multicolumn{1}{c|}{3- and 4-view} & 5- to 8-view & \multicolumn{1}{c|}{All}     & \multicolumn{1}{c|}{3- and 4-view} & 5- to 8-view \\ \cline{2-10} 
\textbf{Baseline}     & \multicolumn{1}{c|}{5.1}  & \multicolumn{1}{c|}{5.82}          & 4.47         & \multicolumn{1}{c|}{5.13}    & \multicolumn{1}{c|}{5.64}          & 4.69         & \multicolumn{1}{c|}{5.2}     & \multicolumn{1}{c|}{5.75}          & 4.72         \\
\textbf{Basic}        & \multicolumn{1}{c|}{4.97} & \multicolumn{1}{c|}{5.07}          & 4.88         & \multicolumn{1}{c|}{5.05}    & \multicolumn{1}{c|}{5.18}          & 4.94         & \multicolumn{1}{c|}{5.23}    & \multicolumn{1}{c|}{5.5}           & 5            \\
\textbf{Partial}      & \multicolumn{1}{c|}{5.12} & \multicolumn{1}{c|}{5}             & 5.22         & \multicolumn{1}{c|}{5.1}     & \multicolumn{1}{c|}{5.04}          & 5.16         & \multicolumn{1}{c|}{5.38}    & \multicolumn{1}{c|}{5.39}          & 5.38         \\
\textbf{Full}         & \multicolumn{1}{c|}{5.45} & \multicolumn{1}{c|}{5.68}          & 5.25         & \multicolumn{1}{c|}{5.33}    & \multicolumn{1}{c|}{5.61}          & 5.09         & \multicolumn{1}{c|}{5.67}    & \multicolumn{1}{c|}{5.93}          & 5.44         \\
\textbf{Origin}       & \multicolumn{1}{c|}{5.55} & \multicolumn{1}{c|}{5.29}          & 5.78         & \multicolumn{1}{c|}{5.58}    & \multicolumn{1}{c|}{5.29}          & 5.84         & \multicolumn{1}{c|}{5.62}    & \multicolumn{1}{c|}{5.21}          & 5.97         \\ \hline
\multicolumn{1}{l|}{} & \multicolumn{3}{c|}{\textbf{Interaction Logic}}                               & \multicolumn{3}{c|}{\textbf{Interaction Helpful to Explore}}                     & \multicolumn{3}{c}{\textbf{Overall}}                                             \\ \hline
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{All}  & \multicolumn{1}{c|}{3- and 4-view} & 5- to 8-view & \multicolumn{1}{c|}{Basic}   & \multicolumn{1}{c|}{3- and 4-view} & 5- to 8-view & \multicolumn{1}{c|}{Basic}   & \multicolumn{1}{c|}{3- and 4-view} & 5- to 8-view \\ \cline{2-10} 
\textbf{Baseline}     & \multicolumn{1}{c|}{3.6}  & \multicolumn{1}{c|}{3.96}          & 3.28         & \multicolumn{1}{c|}{3.53} & \multicolumn{1}{c|}{3.86}          & 3.25         & \multicolumn{1}{c|}{4.37} & \multicolumn{1}{c|}{4.82}          & 3.97         \\
\textbf{Basic}        & \multicolumn{1}{c|}{5.43} & \multicolumn{1}{c|}{5.79}          & 5.13         & \multicolumn{1}{c|}{5.43}    & \multicolumn{1}{c|}{5.75}          & 5.16         & \multicolumn{1}{c|}{5.17}    & \multicolumn{1}{c|}{5.43}          & 4.94         \\
\textbf{Partial}      & \multicolumn{1}{c|}{5.82} & \multicolumn{1}{c|}{5.93}          & 5.72         & \multicolumn{1}{c|}{5.83}  & \multicolumn{1}{c|}{5.89}          & 5.78         & \multicolumn{1}{c|}{5.33}  & \multicolumn{1}{c|}{5.32}          & 5.34         \\
\textbf{Full}         & \multicolumn{1}{c|}{5.82} & \multicolumn{1}{c|}{6.04}          & 5.63         & \multicolumn{1}{c|}{5.87}    & \multicolumn{1}{c|}{5.96}          & 5.78         & \multicolumn{1}{c|}{5.43}    & \multicolumn{1}{c|}{5.71}          & 5.19         \\
\textbf{Origin}       & \multicolumn{1}{c|}{5.32} & \multicolumn{1}{c|}{4.86}          & 5.72         & \multicolumn{1}{c|}{5.28}    & \multicolumn{1}{c|}{4.96}          & 5.56         & \multicolumn{1}{c|}{5.25}    & \multicolumn{1}{c|}{4.86}          & 5.59         \\ \hline
\end{tabular}
\end{table*}
